Reinforcement Learning with Fast Stabilization in Linear Dynamical Systems

In this work, we study model-based reinforcement learning (RL) in unknown stabilizable linear dynamical systems. When learning a dynamical system, one needs to stabilize the unknown dynamics in order to avoid system blow-ups. We propose an algorithm that certifies fast stabilization of the underlying system by effectively exploring the environment with an improved exploration strategy. We show that the proposed algorithm attains $\tilde{\mathcal{O}}(\sqrt{T})$ regret after $T$ time steps of agent-environment interaction. We also show that the regret of the proposed algorithm has only a polynomial dependence in the problem dimensions, which gives an exponential improvement over the prior methods. Our improved exploration method is simple, yet efficient, and it combines a sophisticated exploration policy in RL with an isotropic exploration strategy to achieve fast stabilization and improved regret. We empirically demonstrate that the proposed algorithm outperforms other popular methods in several adaptive control tasks.

==> relatedworks.tex <==
\section{Related Work}
% \textbf{Asymptotic results in adaptive control:} Over the last decade, a large body of literature address the controlling and minimizing costs in unknown dynamical systems. The classical learning-based methods provide fundamental asymptotic convergence guarantees~\citep{lai1982least,lai1987asymptotically, fiechter1997pac}. They show that as the number of interactions increase, the gap between a proposed policy and the optimal one closes. 
\textbf{Finite-time regret guarantees:} Prior works study the problem of regret minimization in \LQR{}s and achieve sublinear regret using CEC{}s \citep{mania2019certainty, faradonbeh2018input,faradonbeh2020adaptive}, robust controllers \citep{dean2018regret}, the \OFU principle \citep{abeille2020efficient}, Thompson sampling 
\citep{abeille2018improved,ouyang2017learning} and an SDP relaxation \citep{cohen2019learning} with a lower bound provided in \citet{simchowitz2020naive}. The main common feature of these works is that they all assume a given initial stabilizing policy and do not design autonomous learning agents which is the main focus of this paper.  


\textbf{Finite time guarantees for finding a stabilizing controller:} Similar to the regret minimization, there has been a growing interest in finite-time stabilization of linear dynamical systems \citep{dean2019sample,faradonbeh2018finite,faradonbeh2019randomized}. Among these works \citet{faradonbeh2018finite} is the closest to our work. However, there are significant differences in the methods and the span of our results. In \citet{faradonbeh2018finite}, random linear controllers are used solely for finding a stabilizing set without a control goal. This results in the explosion of state, presumably exponentially in time, leading to a regret that scales exponentially in exploration time. Even though it provides many insightful aspects for finding a stabilizing set in finite-time, it does not provide a cost analysis of this process or an adaptive control policy. Moreover, the stabilizing set in \citet{faradonbeh2018finite} is somewhat implicit. It relates to the minimum value that satisfies a specific condition for the roots of a polynomial.
This results in an implicit sample complexity for constructing such a set. On the other hand, in this work, we provide a complete study of an autonomous learning algorithm for the online \LQR problem. Among our results we give an explicit formulation of the stabilizing set and a sample complexity that only relates to the minimal stabilizability information of the system.

% \textbf{\OFU based works:} For control problems, \OFU principle was first used by \citet{campi1998adaptive}. Besides adaptive control of \LQR, \OFU principle is widely used in a variety of decision making paradigm, such as multi-arm bandit~\citep{auer2002using}, linear bandit~\citep{abbasi2011improved}, Markov Decision Processes~\citep{jaksch2010near,azizzadenesheli2016reinforcement}, and adaptive control of partially observable linear quadratic control systems~\citep{lale2020regret,lale2020root}. Recently, \cite{abeille2020efficient} provide computationally feasible optimism in the face uncertainty approach for large dimensional \LQR{}s. However, they assume access to a stabilizing set in the beginning of the algorithm where the regret of obtaining such set or its effect on the state is not analyzed.

\textbf{Online \LQR problem with adversarial disturbances:} 
% Besides the standard setting of online \LQR problem considered in this paper, there are various works that consider more general settings. One line of research considers the partially observable counterpart of \LQR termed as \LQG. It is the setting where instead of exact state vector, a noisy linear combination of the state vector is observed. In this setting \citet{mania2019certainty, simchowitz2020improper, lale2020root} achieve $\sqrt{T}$ regret and \citet{lale2020logarithmic} introduces the algorithm that achieves first polylogarithmic regret in this setting. 
Another line of research considers online \LQR problem under adversarial disturbances \citep{hazan2019nonstochastic, simchowitz2020improper,chen2020black}. These works either assume a given stabilizing controller or open-loop stable system dynamics, except \citet{chen2020black}. Independently and concurrently, the recent work by \citet{chen2020black} designs an autonomous learning algorithm and regret guarantees that are similar to the current work. However, the approaches and the settings have major differences. \citet{chen2020black} considers the restrictive setting of \textit{controllable} systems yet with general adversarial disturbances and general cost functions. They inject \textit{significantly} big inputs, \textit{exponential in system parameters}, with a pure exploration intent guarantee recovery of system parameters and stabilization. This negatively affects the practicality of the algorithm. On the other hand, in this work, we inject isotropic Gaussian perturbations to improve the exploration in the stochastic (general sub-Gaussian noise) \textit{stabilizable} system while still aiming to control, \textit{i.e.} no pure exploration phase. Interestingly, both of these works attain exponential dependency in system parameters in their corresponding stabilization phases. 

